Edge-preserving noise for diffusion models

Classical diffusion models typically rely on isotropic Gaussian noise, treating all regions uniformly and overlooking structural information important for high-quality generation. We introduce an edge-preserving diffusion process that generalizes isotropic models via a hybrid noise scheme with an edge-aware scheduler that smoothly transitions from edge-preserving to isotropic noise. This enables the model to capture fine structural details while generally maintaining global performance. We evaluate the impact of structure-aware noise in both diffusion and flow-matching frameworks, and show that existing isotropic models can be efficiently fine-tuned with edge-preserving noise, making our framework practical for adapting pre-trained systems. Beyond unconditional generation, our method particularly shows improvements in structure-guided tasks such as stroke-to-image synthesis, improving robustness and perceptual quality, as evidenced by consistent improvements across FID, KID, and CLIP-score.

==> figures/ablation.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{0.71}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\hspace{0.1cm} \scriptsize \citet{heitz2023iterative}}
% FID: $\textbf{35.71}$ & - & - & -
  &   &   %&  
\\
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_lambda/aniso_church_res128_kmin1e-05_kmax0.1_pt0.5_00000003.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_lambda/aniso_church_res128_kmin0.01_kmax0.01_pt0.5_00000003.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_lambda/aniso_church_res128_kmin0.0001_kmax0.0001_pt0.5_00000003.png}
\end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_lambda/aniso_church_res128_kmin1e-06_kmax1e-06_pt0.5_00000003.png}
% \end{tikzpicture}
\\
$\EdgeSensitivityTimeVarying$: linear & $\EdgeSensitivityTimeVarying:1e^{-2}$ & $\EdgeSensitivityTimeVarying:1e^{-4}$ %& $0.000001$
\\
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.025cm}
\vline width 0.7 pt
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{}}
FID: $23.91$ & $\textbf{22.11}$ & $33.06$
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_tau/tau_0.25.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_tau/tau_0.5.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_tau/tau_0.75.png}
\end{tikzpicture}
\\[-0.4mm]
$\TransitionPt$: $0.25$ & $0.5$ (Ours) & $0.75$
\\[-0.4mm]
\end{tabular}
\end{tabular}

\begin{tabular}{c@{\;}c@{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.025cm}
% \vline width 0.7 pt
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{}}
FID: $18.01$ & $21.23$ & $\textbf{13.06}$
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/sigmoid.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/cosine.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/linear.png}
\end{tikzpicture}
\\[-0.4mm]
$\TransitionFn$: Sigmoid & Cosine & \textbf{Linear}
\\[-0.4mm]
\end{tabular}
\end{tabular}

==> figures/ablation_trans_fn.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{0.71}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.025cm}
% \vline width 0.7 pt
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{}}
FID: $18.01$ & $21.23$ & $\textbf{13.06}$
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/sigmoid.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/cosine.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{ablation_trans_fns/linear.png}
\end{tikzpicture}
\\[-0.4mm]
$\TransitionFn$: Sigmoid & Cosine & \textbf{Linear}
\\[-0.4mm]
\end{tabular}
\end{tabular}


==> figures/comparison_fm.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageNonSquared}[1]{%
    % \begin{tikzpicture}[scale=1.2]
        \begin{scope}
            \clip (0,0) -- (4,0) -- (4,2) -- (0,2) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (4cm,2cm);
        \end{scope}
        \draw (0,0) -- (4,0) -- (4,2) -- (0,2) -- cycle;
        
    % \end{tikzpicture}%
}



% \newcommand{\PlotSingleImageWithLine}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%         \draw[dashed] (0, -0.13) -- (2.5, -0.13);
%     % \end{tikzpicture}%
% }


% \newcommand{\TwoColumnFigure}[2]{%
%     \begin{tabular}{c@{\;}c@{}}
%         \hspace*{-2.5mm}
%         \begin{tikzpicture}[scale=0.563]
%             \PlotSingleImage{#1}
%         \end{tikzpicture}
%          & 
%          \begin{tikzpicture}[scale=0.563]
%             \PlotSingleImage{#2}
%         \end{tikzpicture}
%     \end{tabular}%
% }


% define the scale value and use it for all
\newcommand\scalevalue{1.0}    % 0.65, 1.85

%
% \small
\hspace*{-6.0mm}
\begin{tabular}{c@{\;}c@{\;}c@{}}


\begin{tabular}{c@{\;}c@{}}

\\[-0.4mm]
\scriptsize EP-OT-FM (Ours) FID/KID: 6.50/0.0028 \\
\scriptsize OT-FM FID/KID: 6.38/0.0027
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cat_128/1.png}
\end{tikzpicture}
\\[-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cat_128/2.png}
\end{tikzpicture}
\\ [-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cat_128/3.png}
\end{tikzpicture}

\\[-0.4mm]
AFHQ-Cat ($128^2$)
\\[-0.4mm]
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{c@{\;}c@{}}

\\[-0.4mm]
\scriptsize EP-OT-FM (Ours) FID/KID: 5.89/0.005 \\
\scriptsize OT-FM FID/KID: 5.84/0.005
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/celeba_64/1.png}
\end{tikzpicture}
\\[-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/celeba_64/2.png}
\end{tikzpicture}
\\ [-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/celeba_64/3.png}
\end{tikzpicture}

\\[-0.4mm]
CelebA ($64^2$) 
\\[-0.4mm]
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{c@{\;}c@{}}
\\[-0.4mm]
\scriptsize EP-OT-FM (Ours) FID/KID: 3.16/0.0008 \\
\scriptsize OT-FM FID/KID: 3.14/0.0008
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cifar10/1.png}
\end{tikzpicture}
\\[-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cifar10/2.png}
\end{tikzpicture}
\\ [-1mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison_fm/cifar10/3.png}
\end{tikzpicture}

\\[-0.4mm]
CIFAR-10 ($32^2$) 
\\[-0.4mm]
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}


==> figures/comparison_new.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageNonSquared}[1]{%
    % \begin{tikzpicture}[scale=1.2]
        \begin{scope}
            \clip (0,0) -- (4,0) -- (4,2) -- (0,2) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (4cm,2cm);
        \end{scope}
        \draw (0,0) -- (4,0) -- (4,2) -- (0,2) -- cycle;
        
    % \end{tikzpicture}%
}



% \newcommand{\PlotSingleImageWithLine}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%         \draw[dashed] (0, -0.13) -- (2.5, -0.13);
%     % \end{tikzpicture}%
% }


% \newcommand{\TwoColumnFigure}[2]{%
%     \begin{tabular}{c@{\;}c@{}}
%         \hspace*{-2.5mm}
%         \begin{tikzpicture}[scale=0.563]
%             \PlotSingleImage{#1}
%         \end{tikzpicture}
%          & 
%          \begin{tikzpicture}[scale=0.563]
%             \PlotSingleImage{#2}
%         \end{tikzpicture}
%     \end{tabular}%
% }


% define the scale value and use it for all
\newcommand\scalevalue{0.80}    % 0.65, 1.85

%
% \small
\hspace*{-4.0mm}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
\begin{tabular}{c@{\;}c@{}}
% \rotatebox{90}{\hspace{0.2cm} \scriptsize CelebA($128^2$)}
\rotatebox{90}{\hspace{0.15cm} \scriptsize Cat ($128^2$)}
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/cat128/ihdm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/celeba/ihdm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/lsun_church/ihdm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_celeba_res256/ihdm_celeba_res256_grid.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_cat_res512/ihdm_cat_512_grid.png}
\end{tikzpicture}
\\[-0.4mm]
IHDM
\\[-0.4mm]
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vline width 0.7 pt
\begin{tabular}{c@{\;}c@{}}
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/cat128/bndm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/celeba/bndm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/lsun_church/bndm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_celeba_res256/bndm_celeba_res256_grid.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_cat_res512/bndm_cat_512_grid.png}
\end{tikzpicture}
\\[-0.4mm]
BNDM
\\[-0.4mm]
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vline width 0.7 pt
\begin{tabular}{c@{\;}c@{}}
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/cat128/ddpm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/celeba/ddpm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/lsun_church/ddpm.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_celeba_res256/ddpm_celeba_res256_grid.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_cat_res512/ddpm_cat_512_grid.png}
\end{tikzpicture}
\\[-0.4mm]
DDPM
\\[-0.4mm]
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vline width 0.7 pt
\begin{tabular}{c@{\;}c@{}}
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/cat128/ours.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/celeba/ours.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{comparison/lsun_church/ours.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_celeba_res256/ours_celeba_res256_grid.png}
\end{tikzpicture}
\\[-0.4mm]
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageNonSquared{ldm_cat_res512/ours_cat_512_grid.png}
\end{tikzpicture}
\\[-0.4mm]
Ours
\\[-0.4mm]
\end{tabular}
\end{tabular}


==> figures/human_sketch_dataset_small.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{1.0}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\hspace{0.1cm} \scriptsize \citet{heitz2023iterative}}
% FID: $\textbf{35.71}$ & - & - & -
   % & - & -  &  \textbf{39.04} & 40.95  & 68.0
% \\
\rotatebox{90}{\hspace{-0.1cm} \footnotesize DDPM (FID: 67.97)}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ddpm/1.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ddpm/2.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ddpm/3.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ddpm/5.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ddpm/6.png}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{-0.1cm} \footnotesize	\textbf{Ours (FID: 40.03)}}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ours/6.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ours/2.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ours/3.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ours/4.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{human_sketch_dataset/ours/5.png}
\end{tikzpicture}
\\
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hspace{0.025cm}
% \vline width 0.7 pt
% \footnotesize
% \begin{tabular}{c@{\;}c@{\;}c@{}}
% FID: $23.91$ & $\textbf{22.11}$ & $33.06$
% \\[-0.4mm]
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.25.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.5.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.75.png}
% \end{tikzpicture}
% \\[-0.4mm]
% $\TransitionPt$: $0.25$ & $0.5$ (Ours) & $0.75$
% \\[-0.4mm]
% \end{tabular}
\end{tabular}



==> figures/sde_edit_comparison_cat.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{1.0}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\hspace{0.1cm} \scriptsize \citet{heitz2023iterative}}
% FID: $\textbf{35.71}$ & - & - & -
   & - & -  &  \textbf{17.03} & 18.92  & -
\\
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{sde_edit_comparison/cat/original_image.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{sde_edit_comparison/cat/stroke_painting_from_image.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{sde_edit_comparison/cat/ours_generated.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{sde_edit_comparison/cat/ddpm_generated.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{sde_edit_comparison/cat/bndm_generated.png}
\end{tikzpicture}
\\
&Original & Stroke painting & Ours & DDPM & BNDM
\\
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hspace{0.025cm}
% \vline width 0.7 pt
% \footnotesize
% \begin{tabular}{c@{\;}c@{\;}c@{}}
% FID: $23.91$ & $\textbf{22.11}$ & $33.06$
% \\[-0.4mm]
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.25.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.5.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.75.png}
% \end{tikzpicture}
% \\[-0.4mm]
% $\TransitionPt$: $0.25$ & $0.5$ (Ours) & $0.75$
% \\[-0.4mm]
% \end{tabular}
\end{tabular}


==> figures/user_created_stroke_painting.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{0.65}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\hspace{0.1cm} \scriptsize \citet{heitz2023iterative}}
% FID: $\textbf{35.71}$ & - & - & -
\\
&
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{user_created_stroke_guide/cat/original.png}
% \end{tikzpicture}
% &
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/cat/stroke_painting.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/cat/ours.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/cat/ddpm.png}
\end{tikzpicture}
\\
&
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{user_created_stroke_guide/church/original.png}
% \end{tikzpicture}
% &
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/stroke_painting.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/ours.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/ddpm.png}
\end{tikzpicture}
\\
% &Original 
& Hand-drawn & Ours & DDPM \\
& & painting & & 
\\
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hspace{0.025cm}
% \vline width 0.7 pt
% \footnotesize
% \begin{tabular}{c@{\;}c@{\;}c@{}}
% FID: $23.91$ & $\textbf{22.11}$ & $33.06$
% \\[-0.4mm]
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.25.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.5.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.75.png}
% \end{tikzpicture}
% \\[-0.4mm]
% $\TransitionPt$: $0.25$ & $0.5$ (Ours) & $0.75$
% \\[-0.4mm]
% \end{tabular}
\end{tabular}


==> figures/user_created_stroke_painting_church.tex <==
%!TEX root = ../EGauthorGuidelines-conf-sub.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}


\newcommand{\PlotSingleImageWithLine}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        \draw[dashed] (0, -0.13) -- (2.5, -0.13);
    % \end{tikzpicture}%
}


\newcommand{\TwoColumnFigure}[2]{%
    \begin{tabular}{c@{\;}c@{}}
        \hspace*{-2.5mm}
        \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#1}
        \end{tikzpicture}
         & 
         \begin{tikzpicture}[scale=0.563]
            \PlotSingleImage{#2}
        \end{tikzpicture}
    \end{tabular}%
}
% define the scale value and use it for all
\newcommand\scalevalue{1.0}    % 0.65

%
% \small
\hspace*{-5mm}
\begin{tabular}{c@{\;}c@{}}
\footnotesize
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{\;}c@{}}

% \rotatebox{90}{\hspace{0.1cm} \scriptsize \citet{heitz2023iterative}}
% FID: $\textbf{35.71}$ & - & - & -
\\
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/original.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/stroke_painting.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/ours.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{user_created_stroke_guide/church/ddpm.png}
\end{tikzpicture}
\\
&Original & Hand-drawn painting & Ours & DDPM 
\\
\end{tabular}
&
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hspace{0.025cm}
% \vline width 0.7 pt
% \footnotesize
% \begin{tabular}{c@{\;}c@{\;}c@{}}
% FID: $23.91$ & $\textbf{22.11}$ & $33.06$
% \\[-0.4mm]
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.25.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.5.png}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{ablation_tau/tau_0.75.png}
% \end{tikzpicture}
% \\[-0.4mm]
% $\TransitionPt$: $0.25$ & $0.5$ (Ours) & $0.75$
% \\[-0.4mm]
% \end{tabular}
\end{tabular}

